FireRedTTS: A Foundation Text-To-Speech Framework for Industry-Level Generative Speech Applications

This work proposes FireRedTTS, a foundation text-to-speech framework, to meet the growing demands for personalized and diverse generative speech applications. The framework comprises three parts: data processing, foundation system, and downstream applications. First, we comprehensively present our data processing pipeline, which transforms massive raw audio into a large-scale high-quality TTS dataset with rich annotations and a wide coverage of content, speaking style, and timbre. Then, we propose a language-model-based foundation TTS system. The speech signal is compressed into discrete semantic tokens via a semantic-aware speech tokenizer, and can be generated by a language model from the prompt text and audio. Then, a two-stage waveform generator is proposed to decode them to the high-fidelity waveform. We present two applications of this system: voice cloning for dubbing and human-like speech generation for chatbots. The experimental results demonstrate the solid in-context learning capability of FireRedTTS, which can stably synthesize high-quality speech consistent with the prompt text and audio. For dubbing, FireRedTTS can clone target voices in a zero-shot way for the UGC scenario and adapt to studio-level expressive voice characters in the PUGC scenario via few-shot fine-tuning with 1-hour recording. Moreover, FireRedTTS achieves controllable human-like speech generation in a casual style with paralinguistic behaviors and emotions via instruction tuning, to better serve spoken chatbots.

==> table/asr_compare.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{cccc}
\hline
 & \textbf{Video($\downarrow$)} & \textbf{Live($\downarrow$)} & \textbf{Message($\downarrow$)} \\ \hline \hline
\textbf{RedASR} & \textbf{5.5} & \textbf{4.8} & \textbf{6.9} \\
FunASR & 8.7 & 6.5 & 7.9 \\ \hline
\end{tabular}
\caption{Comparison of transcription WER between RedASR and publicly available FunASR across three different speech sources.}
\label{tab:asr_compare}
\end{table}



==> table/exp_content_consistency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\begin{tabular}{c|ccc|c}
\hline
\multirow{2}{*}{\textbf{System}} & \multicolumn{3}{c|}{\textbf{SER(\%)($\downarrow$)}}                                              & \multirow{2}{*}{\textbf{SMOS($\uparrow$)}} \\ \cline{2-4}
                                 & \multicolumn{1}{c|}{\textbf{ZH}} & \multicolumn{1}{c|}{\textbf{EN}} & \textbf{MIX} &                                \\ \hline
GroundTruth                      & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & -            & 4.53                           \\
CocyVoice                        & \multicolumn{1}{c|}{6.94}        & \multicolumn{1}{c|}{13.83}       & 33.00        & 4.15                           \\
Ours                             & \multicolumn{1}{c|}{2.09}        & \multicolumn{1}{c|}{12.00}       & 8.50         & 4.32                           \\ \hline
\end{tabular}
\caption{The comparison of our system and CosyVoice generated speeches on the test set in terms of Sentence error rate (SER) and SMOS.}
\label{tab:exp_content_consistency}
\end{table}

==> table/exp_decoder.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\begin{tabular}{c|ccc|c}
\hline
\multirow{2}{*}{\textbf{System}} & \multicolumn{3}{c|}{\textbf{SER(\%)($\downarrow$)}}                                              & \multirow{2}{*}{\textbf{SMOS($\uparrow$)}} \\ \cline{2-4}
                                 & \multicolumn{1}{c|}{\textbf{ZH}} & \multicolumn{1}{c|}{\textbf{EN}} & \textbf{MIX} &                                \\ \hline
GroundTruth                      & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & -            & 4.53                           \\
CocyVoice                        & \multicolumn{1}{c|}{6.94}        & \multicolumn{1}{c|}{13.83}       & 33.00        & 4.15                           \\
Ours                             & \multicolumn{1}{c|}{2.09}        & \multicolumn{1}{c|}{12.00}       & 8.50         & 4.32                           \\ \hline
\end{tabular}
\caption{The CMOS evaluation}
\label{tab:exp_decoder}
\end{table}

==> table/exp_emotion_control.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccc}
\toprule
\textbf{System} & \textbf{Happy} & \textbf{Sad} & \textbf{Angry} \\ \hline
base & 0.76 & 0.96 & 0.83 \\
\hspace{3mm}+ finetuned & 0.76 & 0.96 & 0.83 \\ \bottomrule
\end{tabular}
\caption{Comparison of emotion control accuracy after finetuning.}
\label{tab:exp_emotion_control}
\end{table}

==> table/exp_spon_naturalness.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lc}
\toprule
\textbf{System} & \textbf{Naturalness MOS} \\ \hline
baseline & x \\
\hspace{3mm}+ emotion control & x \\ 
\hspace{3mm}+ spontaneous label control & x \\ 
\hspace{3mm}+ both & x \\ \bottomrule
\end{tabular}
\caption{Naturalness MOS of systems with 95\% confidence intervals.}
\label{tab:exp_spon_naturalness}
\end{table}

==> table/exp_voiceclone_crosslingual.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cccc}
\toprule
\textbf{Prompt Language} & \textbf{Text Language} & \textbf{MOS} & \textbf{Speaker Similarity(\%)} \\ \hline
\multirow{2}{*}{Mandarin} & Mixed & 4.77 & 72.87\% \\
 & English & 4.36 & 63.42\% \\ \hline
\multirow{2}{*}{English} & Mandarin & 4.20 & 62.28\% \\
 & Mixed & 4.16 & 62.77\% \\ \bottomrule
\end{tabular}
\caption{Voice cloning performance in cross-lingual settings.}
\label{tab:exp_vc_crosslin}
\end{table}

==> table/exp_voiceclone_fewshot.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{ccc}
\toprule
 & \textbf{MOS$(\uparrow)$} & \textbf{SIM(\%)($\uparrow$)} \\ \hline
zeroshot & 4.25 & 73.61 \\
fewshot 2min & 4.31 & 73.85 \\ \bottomrule
\end{tabular}
\caption{Voice cloning under zero-shot and few-shot conditions for UGC scenario.}
\label{tab:exp_vc_fewshot}
\end{table}

==> table/pipeline_funnel.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{ccc}
\hline
 & \textbf{Total Duration(h)} & \textbf{Remain(\%)} \\ \hline \hline
Original & 260.3k & 100\% \\ \hline
Enhancement & 260.3k & 100\% \\
VAD & 245.2k & 94.22\% \\
Speaker Clustering & 220.9k & 84.88\% \\
Quality Filtering & 111.8k & 42.95\% \\ \hline
\end{tabular}
\caption{Amount of speech data remaining after each processing step.}
\label{tab:pipeline_funnel}
\end{table}



==> table/spon_label.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{ccc}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Spontaneous\\ behaviors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Text token \\ format\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Spontaneous\\ labels\end{tabular}} \\ \midrule
Filled pause & \chn{嗯} & 0 \\
Char repetition & \chn{我我} $[\text{hic}]$ & 0 \\
Word repetition & \chn{就是就是} $[\text{rep}]$ & 0 \\
Breath & $[\text{breath}]$ & 0 \\
Laugh & $[\text{laugh}]$ & 1 \\
Laugh while talk & \chn{哈哈哈} & 1 \\
Emphasis & \chn{嗯} & 2 \\ 
\bottomrule
\end{tabular}
\caption{Spontaneous behaviors, their corresponding text token input formats, and spontaneous labels.}
\label{tab:spon_label}
\end{table}


==> table/vad_compare.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{cccc}
\hline
 & \textbf{Accuracy($\uparrow$)} & \textbf{F1($\uparrow$)} & \textbf{RTF($\downarrow$)} \\ \hline \hline
\textbf{Red VAD} & \textbf{0.888} & \textbf{0.920} & 0.0066 \\
FunASR VAD & 0.811 & 0.863 & 0.0163 \\ \hline
\end{tabular}
\caption{Comparison between RedVAD, FunASR VAD, and PyDub VAD in terms of accuracy, F1 score and real-time-factor(RTF).}
\label{tab:vad_compare}
\end{table}
